Diversify Your Datasets: Analyzing Generalization via Controlled Variance in Adversarial Datasets

Phenomenon-specific "adversarial" datasets have been recently designed to perform targeted stress-tests for particular inference types. Recent work (Liu et al., 2019a) proposed that such datasets can be utilized for training NLI and other types of models, often allowing to learn the phenomenon in focus and improve on the challenge dataset, indicating a "blind spot" in the original training data. Yet, although a model can improve in such a training process, it might still be vulnerable to other challenge datasets targeting the same phenomenon but drawn from a different distribution, such as having a different syntactic complexity level. In this work, we extend this method to drive conclusions about a model's ability to learn and generalize a target phenomenon rather than to "learn" a dataset, by controlling additional aspects in the adversarial datasets. We demonstrate our approach on two inference phenomena - dative alternation and numerical reasoning, elaborating, and in some cases contradicting, the results of Liu et al.. Our methodology enables building better challenge datasets for creating more robust models, and may yield better model understanding and subsequent overarching improvements.

==> backup.tex <==
This is a binary classification for the learning ability of the challenge (EP in our case). it can either learn it or not. To give a context to our probing method, we divide the probing task to 3 degrees:

\begin{enumerate}
    \item 1st degree Probing (Poliak - which paper?) - probing for a phenomenon after training on MNLI. Let's take the Dative Alternation EP (DAEP) as a running example. In this probing type, we'll get a 0\% accuracy (on the contradiction template).
    
    \item 2nd degree probing \cite{liu2019inoculation} - for failure in 1st degree probing (i.e. challenge dataset) , see if model can learn the phenomena after fine-tuning: If so, it's the dataset's blind spot; if not - it's the model's weakness. For the DAEP, we'll see that we only get to 45\% accuracy after fine-tuning on the DAEP dataset.
    
    \item 3rd degree probing (Generalization, this paper) - for failure in 2nd degree probing (i.e. model's weakness) see over what axis the model fails to generalize (Syntactic, lexical, EP-specific, etc.). For DAEP, we might see that for a given syntax structure, the model can only generalize for sentences with exactly the same depth of the dative verb in the constituent parse tree, but can generalize to any type of dative verb and to any lexical distribution (vered, this example is only for you ... I'll think of a better one...). For Hypernymy EP we might notice that the model is syntax agnostic, but can't generalize from one hypernymy class to another.
\end{enumerate}

We can look at the 3rd degree probing from a different angle - for a given dataset with given distributions over a few generalization axis, probe how well the model can generalize to a different data distribution, and therefore, potentially it can  lead to a generic learning ability of the phenomena across different domains (out-of-domain generalization).
From ido - Show exactly on each EP what I can learn using my method that we can't learn with LIU's (or any other methodology).
Application for this analysis:
A method for probing of 3rd degree would enable the community to aim for models with a better generalization capabilities.
When discovering a weakness in the model, once the generalization ability of the model is understood, we'll be able to synthesize data to inoculate it. So in the example of the DAEP, we'll be able to generate training examples for all depths exist in the test set.

In addition, \newcite{liu2019inoculation} did his probing with non-contextual model and not for EPs as we define it here
When probing a model for different EPs it's very challenging to get enough data that is distributed similarly to the original dataset. Thus, it's important to understand the generalization capability of the model. The stronger this capability is, the less data we need.

To demonstrate our methodology, we base our choice of EPs on the Diagnostic dataset of GLUE \cite{wang2018glue}. We analyze the generalization capacity of two EPs as they described at GLUE. 

We chose the spans of the premise template manually in a way that rephrasing the argument will have only little effect on the premise syntax. We used annotators to validate the grammaticality and the coherence of the new sentences created after the instantiations. After the instantiation of all the arguments, although some sentences might hear weird, they are all grammatical and \textit{could} make sense, and are therefore valid for analyzing local phenomena, as opposed to analyzing a summarization task for example.
For each premise we created between 4 to 6 instantiations in addition to the original argument wording. We used all possible combinations of the different arguments to generate hundreds of premises per template. 
For each such new premise, we generated  multiple hypothesis than differ from the premise only in the EP in focus. This enables us to isolate the phenomenon in focus from other phenomena and analyze only the influence of this change. To generate the hypotheses we used different rules relevant for each EP.  

To control the variance between the training and test sets, for each EP we synthetically generate different dataset variants using templates based on premises taken from the MultiNLI training set \cite{N18-1101}. We denote each such premise as \textit{premise template}. We then defined for each premise template 4-7 spans as arguments and asked Mechanical Turk workers to rephrase each such argument separately, leaving the rest of the sentence unchanged, in a way that yields a new grammatical and coherent sentence but with a different meaning that can make sense in some possible made-up context. For example, for the Datives dataset, we took the following Multi-NLI premise and split it in the following way:

 We took 14 dative verbs and looked for Multi-NLI premises where these verbs appear in their dative form with two direct objects. For each verb we sampled two such sentences and created 28 premise templates. For each premise we then created 3 hypotheses as can be seen in our running example:

(4)	Premise: The high school teachers aren't willing to lend \textbf{us} \underline{their air bases}.

(5)	Hypothesis 1 (Entailment): The high school teachers aren't willing to lend \underline{their air bases} to \textbf{us}.

(6)	Hypothesis 2 (Entailment): The high school teachers aren't willing to lend \underline{their air bases}.

(7)	Hypothesis 2 (Contradiction): The high school teachers aren't willing to lend \textbf{us}.


% (1)	Premise: [Even our noble Saudi allies] [aren't willing to] lend [us] [their air bases].

% The four arguments of this template are marked in brackets. Possible instantiation (rephrasing) of the first argument yields the following premise:

% (2)	Premise: \textbf{The high school teachers} aren't willing to lend us their air bases.


% To continue our running example, in order to create hypothesis with Entailment label for the premise in (2) we used the dative alternation rule:

% (3)	Hypothesis: The high school teachers aren't willing to lend their air bases \textbf{to us}.

% Depending on the EP, for each premise template there could be multiple matching hypothesizes with different labels. We further discuss it in the next sub-section.

% (5)	Hypothesis 1 (Entailment): The high school teachers aren't willing to lend \underline{their air bases} to \textbf{us}.

% (6)	Hypothesis 2 (Entailment): The high school teachers aren't willing to lend \underline{their air bases}.

% (7)	Hypothesis 2 (Contradiction): The high school teachers aren't willing to lend \textbf{us}.

% Numerical Reasoning belongs to the Logic category, and refers to reasoning based off of numbers. We looked for Multi-NLI premises with the numbers and for others with the phrases \textit{more than} and \textit{less than}. To keep the same terms across all templates and isolate the phenomenon, for some premises we did slight alternations for the original premise, such as replacing numbers written in words to digits and replacing dollar sign to dollar. We created sentence pairs by replacing the numerical phrase with the number Xp in the original premise to one of the three following options in the hypothesis: Xh; more than Xh; less than Xh, while Xh stands for a random number within the chosen range for the dataset and can be equal, smaller or larger to the number Xp in the premise which is also randomly chosen. For example, let’s take the template I have <more than Xp> dollars in my pocket. For Xp = 2 we generate 3 premises:
% P1: I have had more than 3 drinks tonight.
% P2: I have had less than 3 drinks tonight.
% P3: I have had 3 drinks tonight.
% For each premise we can now generate more hypothesis by switching between the Xp, more than Xp, less than Xp, and by changing Xp to Xh<Xp, Xh=Xp and Xh>Xp. Overall, we generated 22 different entailment pairs for each template. For example, for P1 we can now generate the following hypothesizes (among others):


% $H_{1_1}$  I have had less than 3 drinks tonight – Label: contradiction

% $H_{1_2}$  I have had 4 drinks tonight – Label: neutral

% $H_{1_3}$  I have had more than 2 drinks tonight – Label: entailment

% The Numerical Reasoning dataset contains 30 sets (9 simple, 12 medium and 9 simple) with 22 template pairs (4 entailment, 6 neutral and 12 contradiction).

% We created sentence pairs by replacing the numerical phrase with the number Xp in the original premise to one of the three following options in the hypothesis: Xh; more than Xh; less than Xh, while Xh stands for a random number within the chosen range for the dataset and can be equal, smaller or larger to the number Xp in the premise which is also randomly chosen. For example, let’s take the template I have <more than Xp> dollars in my pocket. For Xp = 2 we generate 3 premises:
% % P1: I have had more than 3 drinks tonight.
% % P2: I have had less than 3 drinks tonight.
% % P3: I have had 3 drinks tonight.
% % For each premise we can now generate more hypothesis by switching between the Xp, more than Xp, less than Xp, and by changing Xp to Xh<Xp, Xh=Xp and Xh>Xp. Overall, we generated 22 different entailment pairs for each template. For example, for P1 we can now generate the following hypothesizes (among others):


% We created sentence pairs by replacing the numerical phrase with the number Xp in the original premise to one of the three following options in the hypothesis: Xh; more than Xh; less than Xh, while Xh stands for a random number within the chosen range for the dataset and can be equal, smaller or larger to the number Xp in the premise which is also randomly chosen. For example, let’s take the template I have <more than Xp> dollars in my pocket. For Xp = 2 we generate 3 premises:
% % P1: I have had more than 3 drinks tonight.
% % P2: I have had less than 3 drinks tonight.
% % P3: I have had 3 drinks tonight.
% % For each premise we can now generate more hypothesis by switching between the Xp, more than Xp, less than Xp, and by changing Xp to Xh<Xp, Xh=Xp and Xh>Xp. Overall, we generated 22 different entailment pairs for each template. For example, for P1 we can now generate the following hypothesizes (among others):


% The examples generated from the two templates differ only in the verb, and we can therefore understand how well the model generalizes on Datives from one verb seen during training on Datives to an unseen one.

% For example, for the Datives dataset, we took the following Multi-NLI premise and split it in the following way:

% {\bf Generalization Dimensions}:
% For each EP we analyze the generalization capacity over two dimensions: the syntactic complexity dimension, and another EP-specific dimension as detailed in the next sub-section. Our method of generating example from templates allows us to control the syntactic similarity between every two examples. Sampling two examples from the same template ensures high syntactic similarity while examples from different template yields lower similarity which depends on the syntactic similarity between the different premise templates.

% Based on the premise template, we divided each EP dataset into 3 subsets with different syntactic complexity levels: simple, medium and complex according to two criteria: sentence length and \textit{EP depth}. We define EP depth as the depth of the smallest constituency which contains the focus of the EP in the constituency parsing tree of the premise template. For example, for Datives we looked at the depth of the dative verb. For that we used Stanford Parser. We consider examples derived from premise templates shorter than 16 words and with a depth of less than 4 as \textit{simple}, examples longer than 25 words and with depth larger than 6 as \textit{complex}, and the rest as \textit{medium}.

% This split of the EP dataset allows us to test the generalization over the syntactic complexity dimension by training the model on one subset and testing it on another. For example, we can understand if a model can learn an EP on syntactically \textit{simple} examples and generalize it to a \textit{complex} ones.

% For Datives, in addition to the syntactic complexity dimension, we analyze a lexical dimension determined by the dative verb. For each template we create one set of examples with the original verb, and another set using a different verb which was chosen in a way that the new template keeps the sentence coherency. For example, for the template in (1) we changed \textit{lend} with \textit{give}:

% (8)	Premise: [Even our noble Saudi allies] [aren't willing to] \textbf{give} [us] [their air bases].

% For Numerical Reasoning we analyze the dimension of the range of numbers to see how well a model trained on this EP over only a specific range of numbers performs over a test set containing a different range. For that we cloned these 30 sets a twice while limiting the random numbers to distribute only within a specific range for each set. More specifically, we used ranges of 2-999, 100-199 and 200-299. 


We consider examples derived from premise templates shorter than 16 words and with a depth of less than 4 as \textit{simple}, examples longer than 25 words and with depth larger than 6 as \textit{complex}, and the rest as \textit{medium}.

% In this section, we use a pre-trained BERT base-uncased model \cite{devlin2018bert} that was fine-tuned on the Multi-NLI dataset and analyzed its performance with our two phenomena in a few ways. We start by performing two previously studied analysis method on our dataset: (a) probing for each EP, to test how well the model performs on the EP without any EP-specific fine-tuning [probing tasks citations?-if so, I'll add it] and (b) inoculation by fine-tuning \cite{liu2019inoculation}, to test how well the model can learn the EP. We then continue to analyzing the models' generalization capacity over the different dimensions.

% \subsection{Probing}
% To create our probing dataset,  for each EP we randomly sampled 6,000 examples from its complete dataset. We then tested the accuracy of the model on this probing set. The results are shown in Table X. 
% %TBD: to update to 10,000 examples

% \paragraph{Datives Alternation}
% Since in the Datives dataset we only had templates for entailment and contradiction labels, we'll only analyze results for these labels. It can be seen that the Entailment label have very high accuracy as opposed to the Contradiction label that has near zero accuracy. That indicates that the model as pre-trained on MNLI didn't learn the dative phenomena from the Multi-NLI training and that it almost always classifies any dative alternation example as entailment. 

% \paragraph{Numerical Reasoning}
% For Numerical Reasoning we we'll only analyze the average accuracy over all labels [the reason is that I didn't see any point to split it as we did in datives. Not sure if we should note that reason]. It is apparent that the model performs quick bad with 44.6\% on the simple subset and very close to random on medium and complex subsets. This indicates the model didn't learn this EP from fine-tuning on the Multi-NLI.

% \subsection{Inoculation by Fine-Tuning}
% For each EP, we split the dataset into training and test sets 77\% and 22\% respectively in a way that the templates in the test weren't included in the training set. Over a few experiments, we then fine-tuned the model with different number of training examples ranging from 0 to 20,000 [TBD] similarly to Liu. For training BERT, we use Adam with learning rate of 7e-7, \beta$_{\text{1}}$ = 0.9, \beta$_{\text{2}}$ = 0.999, and L2 weight decay of 0.01. We trained and tested using 5-fold cross validation iterations [vered – I'm not sure that's the right way to put it. If we have 9 sets, I did 1..2, 3..4, … 6..8 and then 9..1, so I used a few templates twice which I believe is ok]. Results are in Figure Y.

% \paragraph{Datives Alternations}
% Fine-tuning brings the contradiction hypotheses from almost zero accuracy to an impressive 90\% accuracy. The entailment hypotheses also climb to over 88\%. It is clear from the graphs that the model learns well the Dative Alternation phenomena and achieve an even higher accuracy than on the original dev set (MNLI), which indicates a dataset blind spot for the EPs rather than a model weakness. As expected, we can see that it is easier for the model to learn templates with simpler syntactic structure comparing to the complex ones. Fine-tuning with 5000 examples also decreases the performance on the MNLI development set in about 2\%. We might be able to fix that using a different fine-tuning method [cite TBD].

% \paragraph{Numerical Reasoning}
% Although we notice significant improvement in the accuracy of this EP, even after 5000 [TBD] training examples there is still a gap between the dataset and the Multi-NLP dev accuracy. In addition to the more than 4\% decrease on the Multi-NLI development set accuracy, we can tell that there is a model inherent weakness to learn this type of logic phenomena.
 
\paragraph{Lexical Dimension-}[Vered- maybe we should add parts of it to the method - data split section?] 
We'd like to test the models' generalization capacity over different lexicalities and to isolate it from the syntactic structure. since it's difficult to measure the lexical similarity between different sentences directly,  we conduct two experiments that share the same training set, and their test sets has different distances from the training set over the lexical dimension, and similar syntactic structure both to each other and two the common training set. (Vered- should we add a more formal noting here? Something like Syntax(Train0) ~= Syntax(Test1) = Syntax(Test2), 
Lexical(Train0) - Lexical(Test1) < Lexical(Train0) - Lexical(Test2))

To do so, the two test sets only differ in the main verb. Training set- from each of the 14 templates we take a subset of at least 256 examples using only 4 instantiations per argument, while each template uses a different dative verb. Test sets (81 examples per template): T¬est1 – same templates as the training set with different argument (different words) but with the same main verbs and Test2 – identical to Test1 but with a different main verb. We changed the main verb in a way that all examples keep their coherency and grammaticality.  
Example for identical examples with altered dative verb: 
(Vered, how should we desing this one?)
Test1: Netscape also sent him an explanation
Test2: Netscape also offered him an explanation

Results are in Figure~\ref{fig:generalization_datives}a
Comparing same verb experiments to different verb ones, the model seems to perform almost the same for both tests for all both of sentence complexity. This suggest that for Datives Alternation the model generalizes well over the lexical dimension and more specifically over different main verbs. That is, from training on one verb, the model can learn the dative phenomenon and infer over a similar syntactic structure with a different verb. We can also see that for simple syntactic structures it is easier for the model to generalize comparing to complex ones, as there is a 2\% difference between the Same Verb and Different Verb graphs for the complex comparing to hardly any difference between the simple graphs (Vered - 0.85\% - but this is obviously noise). Since we moved on the lexical axis with only little change in the performance, this indicates a relatively high generalization capacity for Datives Alternations over different lexicon.

\paragraph{Syntactic Structure Dimension-} to move along the syntactic dimension we use the 3 sub-sets (simple, medium and complex) as described in section 3.3, while simple syntactic structures are closer to each other but far from medium and farther from complex. We conduct two experiments while for each one we train the model on the simple or complex subsets, and test it on all of the three. We also test each model on subset identical to the training set as a baseline. 
Results are in Figure~\ref{fig:generalization_datives}b
It seems that for syntactically simple sentences, the model succeeds to perform well with only little influence of the training set: 93.8\% accuracy when trained on simple and medium and with 95.3\% trained on complex. However, testing over complex sentences the model in significantly influenced by the syntactic complexity of the training set. The more complex the syntax in the training is the better the performance on the complex test set with 77.2\%, 83.2\% and 91.3\% for training on simple, medium and complex respectively. We conclude that the model straggles to generalize between different syntactic levels. Another observation is that to achieve high performance over datasets with both simple or complex lexical structure, it is best to train the model on examples with high syntactical complexity. 

\paragraph{Numerical Reasoning}

\paragraph{Numbers' Range Dimension-}
...
\paragraph{Syntactic Structure Dimension-}
...

Syntactic Structure- Similar to Datives Alternation, we use the 3 sub-sets of syntactic similarity and conduct two experiments, one trained the simple subset and the other on the complex. 
The results are in Figure~\ref{fig:generalization_numbers}a
As opposed to the Datives Alternation, where after 700 training examples we see a big gap opening correlated to the syntactic distance between the training and test sets, in Numerical Reasoning we can see that after enough training examples, around 3000 in our case, all graphs converge to a maximum distance of 5.8\% (62.33\% accuracy for the complex set trained with simple set and 68.14\% for simple set trained with a different simple set). This indicates that for this EP the syntactic distance between the training and the test sets has only little effect on the performance. We conclude that Numerical Reasoning has a good generalization capacity over syntactic structure. We assume the reason for that unlike the Datives case, here there is no effect of the EP on the syntax. Moving from the premise to the hypothesis we only replace the number and possibly add two words. Therefore, the model doesn’t have to understand the syntax in the area of the EP, but only the arithmetic behind it. Yet, even after the convergence point, the gap doesn’t totally disappear, as the generalization over this dimension isn’t perfect [Vered – how would you explain that?] .


Range- We wanted to test the model’s ability to generalize over different ranges of numbers. For that, we trained the model premise-hypothesis pairs while instantiating numbers between 30 and 49 in the templates, and for the test sets we used the ranges: 30-49, 200-299 and 1000-9999, where the first range is identical to the training set, the second is further and the last range is the farthest and differs in two digits from the training set. Similarly to the Lexical Dimension in the Datives, to keep the lexical dimension unchanged between training and test, we split each template into to sub-template, Si1 and Si2 so they both have similar syntax with different words. So for example, if we used Si1 with random numbers between 30-49 in the training set, we’d then use Si2 with the ranges mentioned above in the test set. [Vered – would you give an example, or is it clear enough? Maybe in a separate box? Maybe we should give an example for the generic case of templates and instantiations or arguments as well in section 3?]
Results are in Figure~\ref{fig:generalization_numbers}b
As expected, both graphs of same range between training and test sets perform better that those of a bigger distance over the Range Dimension. We notice that after 3000 training examples the test set with 30-49 range improves significantly, while the two other ranges get to saturation. This indicates a poor generalization capacity over different ranges. We assume that the improvement in the first range is due to partially memorization of the arithmetic relations between the 20 numbers in the range rather then learning the arithmetic rules. 


% Introduction

In the history of the Recognizing Textual Entailment (RTE) task, also known as Natural Language Inference (NLI) \cite{dagan2013recognizing, bowman-etal-2015-large} ,it was common to transform the premise into the hypothesis through a series of entailment-preserving transformations (syntactic, lexical, etc.) \cite{Stern-2012-biutee}, while each transformation used a single Entailment Phenomenon (EP) [Vered- is it accurate?]. Today's neural models don't explicitly address such phenomena, but may instead learn them implicitly from the training data. Yet, recent adversarial datasets \cite{poliak-etal-2018-collecting, naik-etal-2018-stress} designed for probing different EPs, showed that neural models often fail on inferences including phenomena such as semantic relations and negation. 

For models with low probing results on a given EP, \newcite{liu2019inoculation} suggested inoculation by fine-tuning, that is fine-tuning the model on a subset of the EP, which in some cases results in performance similar to the original dataset, but in other cases performance remain poor even after fine-tuning, which indicates a model inherent weakness rather than a blind spot in the dataset . Unsurprisingly, even for EPs revealing a model weakness, testing the EPs on examples identical to those in the training set of this failed inoculation yields near 100\% accuracy (see section 4.3). But when taking test examples that haven’t been see in training, the higher the distance (syntactic, lexical, and other language characteristics) between these examples and those in the training set, the higher the decrease in the model’s performance over them. In this paper we try to understand \textit{why} the accuracy decreases as the distance increases. We claim [Vered – is this good wording?] that this decrease is due to lack in generalization capacity, and the better the model performs on examples more distinct from the training set the higher this capacity is.

Ideally, we’d like to train a model on a few examples from a given EP and the model to generalize it to distinct examples (that might have different syntax, wording, and other language characteristics as well as combinations with other EPs), that distinguish the tested examples from the ones in training. However, since there are endless such permutations, it’s not feasible to train the model on all possible variants of the EP. We’d like it to generalize from only a few training examples to any possible example. We therefore see generalization as a key quality of the model, and we need to understand it well in order to improve models.

In this paper we present a framework for testing the capability of NLI models to handle specific EPs. We generate new sentence pairs for each EP which consist of only this speacific EP. The sentences differ along multiple dimensions (syntactic, lexical, etc.), allowing us to control the differences between the training and test sets.  This enables (1) performing a fine grained analysis of the model’s ability to learn the tested phenomenon; and (2) analyzing to what extent the model can generalize along those dimensions, as opposed to exploiting possible artifacts in the data.

We focus on two EPs, Dative Alternation and Numerical Reasoning, both taken from GLUE diagnostic dataset \cite{wang2018glue}. For each EP, using Multi-NLI sentence-templates we generate a few datasets (see Section 3) with different distances between training and test. We use a standard NLI model based on pre-trained BERT as the underlying representation and train it on Multi-NLI \cite{Williams2017Multi-NLI}. We then fine-tune the model on our datasets, test it on the matching test sets according to different distances, and analyze the resulted learning curves.

Our experiments show that for dative alternations BERT has a high generalization capacity over the lexical dimension but a low capacity over the syntactic one, while for numerical reasoning the model generalizes well over different syntactic structures but fails to generalize over different numbers range. We suggest that adapting our methodology for the broader range of inference types may yield better model analysis and subsequent overarching improvements.

% Background

    Recognizing Textual Entailment (RTE, also known as NLI)  is the task of identifying, given two text fragments, whether one of them can be inferred from the other \cite{Dagan-2005-RTE}. While previous-generation models relied on domain knowledge and lexical resources like WordNet \cite{Heilman:2010:TEM:1857999.1858143, MacCartney:2008:PAM:1613715.1613817}, with the release of SNLI, a large-scale dataset, the focus shifted to neural models. Typically, these models encode the premise and the hypothesis and combine them to a feature vector which is fed into a MLP to make the entailment prediction. The encoding of the two sentences can be independent or dependent (using attention mechanism). These models don't use any external knowledge apart from pre-trained word embeddings \cite{DBLP:journals/corr/abs-1301-3781}. The various entailment phenomena are expected to be learned from the training instances. However, recent work showed that they fail on phenomena or specific examples that don't exist in the training data: \newcite{glockner-etal-2018-breaking} showed that replacing a single word with its synonym or antonym in simple SNLI examples fails the model and \newcite{glockner-etal-2018-breaking,naik-etal-2018-stress} managed to fail the model by making other  manipulation to the original examples pair, such as changing the numbers to test the numerical reasoning inference and adding the words \textit{and false is not true} at the end of the sentence to test the negation phenomena.
    
    Recently, the word embedding paradigm shifted from static to dynamic, context-sensitive word embeddings, such as ELMo \cite{Peters2018Elmo}, BERT \cite{devlin2018bert}, GPT \cite{radford2018improving}). These models are all unsupervised language-models that has been pre-trained on large-scaled datasets and have been used across a broad range of NLP tasks, outperforming the previous state-of-the-art models. They have been shown to capture various types of linguistic knowledge: \newcite{tenney2018what} and \newcite{peters-EtAl:2018:N18-1} showed that CWE come with some knowledge about a few phenomena: \newcite{peters-EtAl:2018:N18-1}  shows that much is incorporated in the CWE vector (POS, constituency, coref). \newcite{tenney2018what} connect an MLP to train and then test the performance over the phenomena (POS, constituency, dependency, NER, SRL, coreference, cause-effect). SOTA NLI models such as BERT and MT-DNN \cite{Liu2019MNLI-SOTA} use Contextual word embedding (CWE) as their underlying representations, basing their architecture on the recently presented Transformers \cite{Vaswani2017Transformer}. 
    
     To test whether dense representations capture a certain linguistic property, multiple Probing tasks has been recently proposed, such as \newcite{Adi2017fine-grained} and \newcite{Conneau2018what-you-can-cram} that probed for properties like sentence length and word order as well as syntactic and semantic ones.  Others focused on specific linguistic properties such as agreement \cite{Giulianelli2018agreement} and tense \cite{bacon-regier-2018-probing}. Some probing tasks focused on NLI models and showed their weaknesses. \newcite{poliak-etal-2018-collecting} presented a collection of datasets designed to probe a few inference phenomena such as NER and sentiment analysis, and \newcite{glockner-etal-2018-breaking} [Vered- we're already mentioned him. is it ok? should we add Max here again?] made stress tests to NLI models using automatically-constructed adversarial examples.
     For this probing purpose, the NLI model is used as a black box and its weights are frozen during the training of the probing task [ Vered- Poliak experimented with and without freezing - does it matter?] . In contrast, fine-tuning the model on the probing task dataset (i.e. updating its weights) allows answering additional questions such as: why the model fails in the task. \newcite{liu2019inoculation} shows that the answer to this question fall into one of three categories: 
     \begin{enumerate}
        \item \textbf{Dataset blind spots} - gap closes after fine-tuning. That suggests the challenge revealed a lack of diversity in the 
        original dataset.
        \item \textbf{Model fundamental weakness} - gap doesn't close. It is unable to adapt to the challenge data distribution even with some exposure.
        \item (Damaging performance on the original test set) - gap closes but with major [can I say that?] decrease in the performance of the original set.
    \end{enumerate}
    
     So for example, adding ``and true is true'' to the sentence confuses the model (Stress Test), but after training on this attack the model adjusts, which indicates a dataset blind spot.[This part repeats what we wrote in the Intro. ] 


% Conclusions

% Outline from Google Doc
We presented a method of studying how well models generalizes a specific entailment phenomenon it learned from training dataset to other examples that distanced from the training set in multiple levels, as opposed to exploiting possible artifacts in the data. Our method  generates examples for a specific EP that differ along multiple dimensions (syntactic, lexical, etc.), enabling to control the differences between the training and test sets. It then fine-tunes models on those examples and compares models’ behaviors between test examples with low and high proximity to the training set. This analysis yields insights into models and their robustness. We applied our method to analyze BERT \cite{devlin2018bert} and the MultiNLI \cite{Williams2017Multi-NLI} dataset focusing on Datives Alternations and Numerical Reasoning and tested their generalization capacities. Our results indicate that the while the model might straggle to generalize over a certain dimension for some phenomena, it can do so successfully for others. 

A natural direction for future work would be to expend our dataset to include many more entailment phenomena that will allow us to conduct a more extensive analysis for models’ generalization capacity. This would allow us to answer two open questions. The first, is how models generalize a combination of multiple phenomena? That is training on a few EPs separately, how well models would perform on examples containing a combination of them all. The second questions is what's the model ability to distinguish between different phenomena exist in the same training example and apply these phenomena separately in test time. Analysis of these questions better represents the real world where premise and hypothesis distinct in a series of entailment transformations as opposed to only one EP that was studied in this paper.

As has been shown in Section 4.3, fine-tuning on each of our EP specific datasets yields a small decrease in the performance of the original dataset. Avoiding this decrease would enable us to potentially improve the original model’s performance and to make it more robust against adversarial attacks by training the model on many EP specific datasets. One option to avoid it would be to try a method similar to the one presented by \cite {kiperwasser2018}, who suggested to schedule a main task and a helper task in a way that optimizes the performance.

